Suggesting Code Edits in Interactive Machine Learning Notebooks Using Large Language Models

Machine learning developers frequently use interactive computational notebooks, such as Jupyter notebooks, to host code for data processing and model training. Jupyter notebooks provide a convenient tool for writing machine learning pipelines and interactively observing outputs, however, maintaining Jupyter notebooks, e.g., to add new features or fix bugs, can be challenging due to the length and complexity of the notebooks. Moreover, there is no existing benchmark related to developer edits on Jupyter notebooks. To address this, we present the first dataset of 48,398 Jupyter notebook edits derived from 20,095 revisions of 792 machine learning repositories on GitHub, and perform the first study of the using LLMs to predict code edits in Jupyter notebooks. Our dataset captures granular details of cell-level and line-level modifications, offering a foundation for understanding real-world maintenance patterns in machine learning workflows. We observed that the edits on Jupyter notebooks are highly localized, with changes averaging only 166 lines of code in repositories. While larger models outperform smaller counterparts in code editing, all models have low accuracy on our dataset even after finetuning, demonstrating the complexity of real-world machine learning maintenance tasks. Our findings emphasize the critical role of contextual information in improving model performance and point toward promising avenues for advancing large language models' capabilities in engineering machine learning code.

==> defs/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
}

\lstset{escapeinside={(*@}{@*)}}

%%%==========


==> defs/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> tables/table-results-cell.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrrr}
\hline
DeepSeek Model & BLEU  & CodeBLEU & EditSim & RougeL \\ \hline
1.3B           & 8.52 & 17.26    & 26.52   & 21.49  \\
6.7B           & 13.30 & 20.49    & 31.01   & 28.05  \\
1.3B-postproc  & 8.59 & 18.12    & 26.64   & 21.66  \\
6.7B-postproc  & 13.44 & 22.06    & 31.23   & 28.30  \\ \hline
1.3B-finetune  & \textbf{25.86} & \textbf{30.55}    & \textbf{46.53}   & \textbf{40.80}  \\ \hline
\end{tabular}
}

==> tables/table-results-file.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrrr}
\hline
DeepSeek Model & BLEU  & CodeBLEU & EditSim & RougeL \\ \hline
1.3B           & 10.75 & 15.39    & 31.78   & 27.23  \\
6.7B           & 11.76 & 15.34    & 34.68   & 30.45  \\
1.3B-postproc  & 10.78 & 17.42    & 31.76   & 27.36  \\
6.7B-postproc  & 11.81 & 18.64    & 34.70   & 30.57  \\ \hline
1.3B-finetune  & \textbf{27.46} & \textbf{45.26}    & \textbf{47.38}   & \textbf{53.13}  \\ \hline
\end{tabular}
}

==> tables/table-split.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|rrrr|rr}
\toprule
Set   & \#Proj & \#File & LOC     & \#Commits & \#$\Delta$Cells & \#$\Delta$Lines \\ \toprule
full  & 792    & 48,398  & 6,636,971 & 20,095     & 508,634                          & 3,336,142                         \\ \hline
train & 536    & 27,515  & 3,510,884 & 12,874     & 308,731                          & 1,899,031                         \\
val   & 76     & 12,469  & 1,988,162 & 3,660      & 116,313                          & 970,452                          \\
test  & 152    & 8,414   & 1,137,925 & 3,561      & 83,590                           & 466,659                          \\ \hline
\end{tabular}
}

==> tables/table-statistics.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|r rrrrr}
\toprule
Name & Avg & Min & Med & 75\% & 90\% & Max \\
\toprule
commit message \#Words & 5.66 & 3 & 5 & 7 & 9 & 72 \\
file \#Token before diff & 1,511.60 & 1 & 593 & 2,092 & 4,191 & 50,451\\
file \#Token after diff & 2,079.28 & 1 & 1,260 & 2,756 & 4,845 & 79,893\\  % 4,845.30
changed cells \#Token before diff & 344.14 & 1 & 1 & 204 & 944 & 30,800\\  % 944.30
changed cells \#Token after diff & 841.14 & 1 & 191 & 947 & 2,437 & 77,597\\  % 2,437.30
\bottomrule
\end{tabular}
}
